Page curves for a family of exactly solvable evaporating black holes

We study the entanglement entropy of a one-parameter family of exactly solvable gravities in the 2-dimensional asymptotically-flat space. The islands and Page curves of eternal, evaporating and bath-removed black holes are investigated. The different theories in this parameter class are identified through field redefinitions which leave the island invariant. The Page transition is found to occur at the first a third of the black hole life time in the evaporating case for this family of solutions. In addition, we consider gluing the equilibrium black hole and the evaporating one along a null trajectory and study the effect of gluing on the islands and Page curves. In the glued space, the island jumps across two different geometries at a certain retarded time. As a result, the Page transition is stretched and split into two separate ones -- the first transition happens when the net entropy generation stops and the second one occurs as the early radiation effectively starts to become purified. Finally, we discuss the issues concerning the inconsistent rates of purification and the paradox related to the state of the radiation.

==> notes.tex <==
\textcolor{blue}{The drop of the entanglement entropy at late times is slower than the initial increase, as shown in Fig.~\ref{fig:page_gen_removal}. This may not seem to be a problem at first sight. but it can be problematic if we compare the middle stage after the first Page time and the final stage after the second Page time. The argument is the following. The black hole evaporates at a constant rate. The initial period represents the Hawking process which the entropy increases from the production of maximally-entangled Hawking pairs across the horizon. The second phase represents the equilibrium between the purification and thermal entropy generation. The thermal field is understood as one side of the thermal field double. In this period, for every outgoing radiation particle escaping the black hole, an equivalent particle from the thermal field must be absorbed by the black hole to keep the black hole of constant mass. This process is an approximation. However, the entanglement entropy of the black hole being constant while particles from the thermal bath falling into the black hole at the same power as the radiation suggests that the newly-emitted Hawking particle must be in maximal entanglement with the early radiation so that the entanglement entropy of the black hole does not increase. This is in a sharp contradiction with what happens after the removal of the bath. With this maximal entanglement of the late and early radiations, the Page curve curve must decrease at least as fast as the increase at the early stage since the the early radiation is at most maximally entangled with the black hole. This raises the issue of the purification rates. One resolution can be that the island calculation is only an upper bound of the Page curve and does not represent how the entropy will actually behaves. Including more islands is equivalent to summing more complicated topologies in the corresponding replica manifolds. Though how to count all the contributions of the saddles is not clear from the gravitational Euclidean path integral, but these higher topologies are suppressed by their genus numbers and it is reasonable to believe that their contribution is small. This is in contradiction with the naive quantum informational interpretation of the Page curve. One can question that the this interpretation is incorrect or if the thermal bath causes the difference. However, the purity of the final stage of evaporation indicates some mechanisms of purification, and attributing the issue to the bath has the consequence that the thermal field significantly influences the generation of Hawking radiation and plays a key role in the mechanism determining the rate of purification.}


\appendix
\section{Specific solutions of RST-BPP model}
\subsection{Vacuum solution}
The asymptotically Minkowski vacuum solution can be obtained by requiring $b=c=M=0$ and that the energy flux in the asymptotically flat coordinates $\sigma^\pm$ defined by $x^\pm=\pm e^{\pm \sigma^\pm}$ vanishes identically, i.e. $t_\pm(\sigma^\pm)=0$. Transforming to the $x^\pm$ coordinates according to the transformation rule Eq.~\eqref{t_transform} gives
\begin{align}
    t_\pm(x^\pm)=-\frac{1}{4(x^\pm)^2}\,.
\end{align}
Setting the vacuum energy condition in Eq.~\eqref{Eq:Omega}, we obtain the geometry of the vacuum solution 
\begin{align}
    \Om=-x^+x^--\frac{1}{4}\log(-x^+x^-)\,.
\end{align}
This solution does not admit radiation as indicated by $t_\pm(\sigma^\pm)=0$. Note that spacetime we are interested in is bounded by $x^+x^-<-\frac{1}{4}$ and $\pm x^\pm>0$ which is required by Eq.~\eqref{Def:Omega}. The boundary of the spacetime is where the dilaton coupling $e^{2\phi}$ becomes strong and the semi-classical approximation breaks down. Near those regions, the quantum gravitational correction becomes large and we do not pretend to have the full quantum mechanical description of it. In the coordinates $\sigma^\pm$ , the geometry is 
\begin{align}
    \Om=e^{-2\phi}+a \phi+\rm{constant}=e^{2\sigma}-\frac{1}{2}\sigma\,,
\end{align}
where \begin{align}
    \sigma\equiv\frac{\sigma^+-\sigma^-}{2}\,.
\end{align}
In the region far away from the boundary points ($\sigma\rightarrow\infty$), $\phi\approx-\sigma$ and the metric is 
\begin{align}
    ds^2=-e^{2\rho-2\sigma}d\sigma^+d\sigma^-\approx -d\sigma^+d\sigma^-\,,
\end{align}
which is the linear dilaton vacuum. When $a=\frac{1}{2}$, the solution is exactly Minkowski space as $ds^2=-d\sigma^+d\sigma^-$, otherwise it is asymptotically flat in the region far away from the boundary. 

\subsection{Eternal black hole}
The eternal black hole solution is given by letting $b=c=t_\pm=0$, which gives
\beq
\Om=-x^+x^-+M\,.
\eeq
To ensure that the singularity lies inside the apparent horizon, we require that $M>\frac{1}{4}$. Because $\Omega$ is the area of the black hole, the location of the apparent horizon is obtained by requiring $\p_+\Om=0$. This equation is equivalent to that following an outgoing light ray, the area stays constant (is not expanding or is just about to shrink), which is the definition of the apparent horizon. For an eternal black hole, the location of the apparent horizon and the event horizon coincides at $x_+x_-=0$. It is easy to check that the energy flux due to the vacuum Casimir energy is
\beq
\p_\pm^2\Omega=-t_\pm=0\,.
\eeq
Near the future null infinity, $-x^+x^-\gg M$. In this case, we return to the asymptotically flat coordinates $x^\pm=\pm e^{\pm \sigma^\pm}$. The metric is flat near the asymptotic null infinity $ds^2\simeq -d\sigma^+ d\sigma^-$. Transforming the energy flux $t_\pm(x^\pm)$ to the flat coordinates gives
\beq
t_\pm(\sigma^\pm)=\frac{1}{4}\,.
\eeq
This suggests that the black hole has an equivalent amount of incoming and outgoing flux which is the feature of the eternal black hole in equilibrium with the bath. The energy flux gives the Hawking temperature 
\beq
T_{\rm BH}=\frac{1}{2\pi}\,,
\eeq
which is a constant during the evaporation.

\subsection{Black hole from collapsing shell}\label{subsub:bhshell}
Consider a shell of matter with the energy-momentum tensor $T_{++}= \frac{M}{x_0^+}\delta(x^+-x_0^+)$ in the Kruskal coordinates. In the regions inside the shell, the solution is required to be back to the vacuum solution. The geometry of the collapsing shell can be computed from Eq.~\eqref{Eq:eom} to be as follows,
\begin{align}
      \Om=-x^+x^--\frac{1}{4}\log(-x^+x^-)-M(x^+-x_0^+)\theta(x^+-x_0^+)\,,
\end{align}
up to a constant which can be determined by considering the endpoints of the evaporation. The apparent horizon ($\p_+\Om=0$) is located at $-x^+(x^-+M)=\frac{1}{4}$, and the vacuum energy is $t_\pm(x^\pm)=-\frac{1}{4(x^\pm)^2}$. Before the $x^+_0$, the (incoming) asymptotically flat coordinates are given by $\pm e^{\pm\sigma^\pm}=x^\pm$. After $x_0^+$, the (outgoing) asymptotically flat coordinates become 
\begin{align}
    x^+=e^{\t\sigma^+}\,, \quad -(x^-+M)=e^{-\t\sigma^-}\,,
\end{align}
and the metric is $ds^2\approx -d\t\sigma^+d\t\sigma^-$. In the outgoing asymptotically flat coordinates, the energy tensor of the radiation can be computed through the Schwarzian transformation \eqref{t_transform}
\begin{align}
    t_+(\t\sigma^+)=0\,,\quad t_-(\t\sigma^-)=\frac{1}{4}-\frac{(x^-+M)^2}{4(x^-)^2}\,.
\end{align}
In the late times $\t\sigma^-\rightarrow\infty$, the coordinate-dependent terms in $t_-(\t\sigma^-)$ vanishes as $x^-+M\rightarrow 0$, the vacuum energy flux only has a constant outgoing component $t_-(\t\sigma^-)=\frac{1}{4}$, which corresponds to a constant temperature $\frac{1}{2\pi}$. Therefore, the black hole has an evaporation time which is approximately $4M$. This time can be calculated exactly considering the dynamics of the black hole. The evaporation process ends when the apparent horizon hits the singularity at $x^-_{\rm int}=\frac{-M}{1-e^{-4M+2}}$. This corresponds to the evaporation time $\t\sigma^-_{\rm int}=4M-\log M$, which is consistent with the approximation from the energy current consideration. The geometry after the apparent horizon hits the singularity can be continuously mapped to a dilaton vacuum through a thunderbolt emission, an instantaneous emanation of some finite amount of energy in the form of radiation. For the BPP model $a=0$, the resulting vacuum geometry has an infinite throat and is geodesic complete, otherwise it is the vacuum solution with a boundary. However, the details near this endpoint and the vacuum geometry will not influence the overall analysis in this paper. 

\subsection{Gluing two geometries}


\begin{figure}[tbh]
\centering
	\includegraphics[width=100mm]{PD_bathremoval.pdf}
	\caption{Sketch of the Penrose diagram for an black hole with thermal bath removed at $x_0^+$. To the left of the null line $x_0^+$, the geometry is identical to that of an eternal black hole or the black hole in equilibrium with the infalling radiation emitted from an external source. ``AH" represents the apparent horizon, ``EH" stands for the event horizon. $J^-$ and $J^+$ represent the past and future null infinity, respectively. After the evaporation, the space returns to the asymptotically flat space with the boundary.}
	\label{fig:Penrose_removal}
\end{figure}

We assume that the black hole has been in equilibrium with the bath until we remove the bath, and the black hole starts to evaporate henceforth. Therefore, in the asymptotically flat coordinates $\sigma^\pm$, there is no incoming radiation after the null line $x^+>x^+_0$ and the outgoing radiation $t_-(\sigma^-)=\frac{1}{4}$ is the same as that of the initial black hole in equilibrium. Transforming back to the $x^\pm$ coordinates, the corresponding boundary conditions are \footnote{Note that we have a sign difference from \cite{Cruz:1996pg} due to different conventions in the equations of motion.}
\begin{gather}
    t_+(x^+)=-\frac{1}{4(x^+)^2}\theta(x^+-x_0^+)\,,\\
    t_-(x^-)=0\,.
\end{gather}
Putting the boundary conditions back to Eq.~\eqref{Eq:Omega}, we have for $x^+>x_0^+$,
\beq
\Om=-x^+(x^-+\Delta)-\frac{1}{4}\left(\log\frac{x^+}{x^+_0}+1\right)+M\,,
\eeq
where $\Delta=-\frac{1}{4x^+_0}$. For $x^+<x_0^+$, the solution for $\Omega$ is the eternal black hole solution. The apparent horizon at $x_0^+$ satisfies the equation $\left.\p_+\Om\right|_{x^+_0} =-x^-=0$ and is glued continuously at $x^+=x_0^+$ with the apparent horizon of the eternal black hole. A discontinuity appears crossing $x_0^+$ from the horizon of the equilibrium black hole geometry to the event horizon of the bath-removed black hole geometry. The event horizon lies inside the apparent horizon for the evaporating black hole as shown in Fig.~\ref{fig:Penrose_removal}. The evaporation process ends when the apparent horizon reaches the singularity, which occurs at
\begin{align}
    x_{\rm int}^-=\frac{1}{4x_0^+}(1-e^{-4(M-1/4)})\quad {\rm or}\quad \t\sigma^-_{\rm int}= 4M+\log(4x^+_0)-1\,,
\end{align}
where coordinates $\{\t\sigma^+,\t\sigma^-\}$ are now the outgoing asymptotically flat coordinates of the bath-removed geometry defined by 
\begin{align}
    x^+=e^{\tilde\sigma^+}\,,\quad x^-+\Delta=-e^{-\tilde\sigma^-}\,.\label{co:out}
\end{align}
Similarly, it can be shown that the endstate of the black hole and the resulting geometry are the same as that in the evaporating black hole case.
